Accuracy Requirements: Assessing the Importance of First Post-Adiabatic Terms for Small-Mass-Ratio Binaries

We investigate the impact of post-adiabatic (1PA) terms on parameter estimation for extreme and intermediate mass-ratio inspirals using state-of-the-art waveform models. Our analysis is the first to employ Bayesian inference to assess systematic errors for 1PA waveforms. We find that neglecting 1PA terms introduces significant biases for the (small) mass ratio $\epsilon \gtrsim 10^{-5}$ for quasi circular orbits in Schwarzschild spacetime, which can be mitigated with resummed 3PN expressions at 1PA order. Moreover, we show that the secondary spin is strongly correlated with the other intrinsic parameters, and it can not be constrained for $\epsilon \lesssim 10^{-5}$. Finally, we highlight the need for addressing eccentric waveform systematics in the small-mass-ratio regime, as they yield stronger biases than the circular limit in both intrinsic and extrinsic parameters.

==> old_tex/table_MCMC.tex <==
%%%%%%%%%%%%%%
\begin{table*}[tbp]
\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
\multicolumn{1}{c|}{$\eps$}                        & \textbf{Model Waveform} & $\Delta \Phi^{(\text{inj})}$ & $\Delta \Phi^{(\text{bf})}$ & $\mathcal{M}^{(\text{inj})}$ & $\mathcal{M}^{(\text{bf})}$ & $\rho^{(\text{inj})}/\rho^{(\text{opt})}$ & $\rho^{(\text{bf})}/\rho^{(\text{opt})}$ & $\log\mathcal{L}^{(\text{inj})}$ & $\log\mathcal{L}^{(\text{bf})}$ \\ \hline\hline
\multirow{6}{*}{$10^{-5}$}                      & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}                     & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}            & \multicolumn{1}{l}{}            \\
                                                & Cir1PA w/o spin         & $0.779$                      & $0.0165$                    & $0.143$                      & $4.497\times 10^{-5}$       & $83.4\%$                                  & $99.9\%$                                 & $-846$                           & -0.250                          \\
                                                & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}                     & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}            & \multicolumn{1}{l}{}            \\
                                                & Cir0PA 1PA-3PN w/o spin & $0.786$                      & $0.00179$                   & $0.163$                      & $4.293 \times 10^{-6}$      & $81.5\%$                                  & $99.8\%$                                 & $-943$                           & -0.0324                         \\
                                                & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}                     & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}            & \multicolumn{1}{l}{}            \\
                                                & Cir0PA w/o spin         & $3.002$                      & $0.00532$                   & $0.889$                      & $2.412 \times 10^{-6}$      & $6.4\%$                                   & $99.8\%$                                 & $-4800$                          & -0.0234                         \\ \hline \hline
\multicolumn{1}{c|}{\multirow{6}{*}{$10^{-4}$}} &                         &                              &                             &                              &                             &                                           &                                          &                                  &                                 \\
\multicolumn{1}{c|}{}                           & Cir1PA w/o spin         & 3.994                        & 0.00702                     & 0.511                        & $8.601 \times 10^{-6}$      & $30.3\%$                                  & $99.9\%$                                 & -5019                            & -0.336                          \\
\multicolumn{1}{c|}{}                           &                         &                              &                             &                              &                             &                                           &                                          &                                  &                                 \\
\multicolumn{1}{c|}{}                           & Cir0PA 1PA-3PN w/o spin & 4.310                        & 0.0179                      & 0.486                        & $1.26 \times 10^{-4}$       & $34.2\%$                                  & $99.9\%$                                 & -4799                            & -0.441                          \\
\multicolumn{1}{c|}{}                           &                         &                              &                             &                              &                             &                                           &                                          &                                  &                                 \\
\multicolumn{1}{c|}{}                           & Cir0PA w/o spin         & 13.093                       & 0.0354                      & 0.653                        & $2.573 \times 10^{-5}$      & $19.0\%$                                  & $99.9\% $                                & -5506                            & -0.122                          \\ \hline \hline
\multirow{6}{*}{$10^{-3}$}&                         & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}        & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}                     & \multicolumn{1}{l|}{}                    & \multicolumn{1}{l|}{}            & \multicolumn{1}{l}{}            \\
                                                & Cir1PA w/o spin         & 4.518                        & 0.00559                     & 0.922                        & $3.643 \times 10^{-6}$      & $3.3 \%$                                  & $99.9\%$                                 & -112938                          & -0.226                          \\
                                                &                         &                              &                             &                              &                             &                                           &                                          &                                  &                                 \\
                                                & Cir0PA 1PA-3PN w/o spin & 4.882                        & 0.0218                      & 0.949                        & $3.443 \times 10^{-5}$      & $3.4 \%$                                  & $99.9\%$                                 & -112827                          & -2.132                          \\
                                                &                         &                              &                             &                              &                             &                                           &                                          &                                  &                                 \\
                                                & Cir0PA w/o spin         & 14.958                       & 0.153                       & 0.938                        & $6.854 \times 10^{-3}$      & $4.9\%$                                   & $99.1\%$                                 & -122173                          & -524.798                        \\
\multicolumn{1}{c|}{}                           &                         &                              &                             &                              &                             &                                           &                                          &                                  &        
\end{tabular}
\caption{Here we present a summary of computed statistics for various mass ratios $\eps = \{10^{-5}, 10^{-4}, 10^{-3}\}$ (first column) when  comparing an injected cir1PA waveform and approximate model templates (second column).  We compute the orbital dephasings~(Eqs.~\ref{eq:dephasing_injected}-\ref{eq:dephasing_recovered_params})  (third and fourth columns); mismatch (Eqs.~\ref{eq:mismatch_injected}-\ref{eq:mismatch_recovered_params})  (fifth and sixth columns);  accumulated SNRs (Eqs.~\ref{eq:accum_SNR_true}-\ref{eq:accum_SNR_bf}) (seventh and eighth columns); and, finally the log-likelihood function, Eq.~\eqref{eq:likelihood_no_noise}, at the injected/recovered parameters. The top, middle, and bottom panels of this table correspond to the top, middle, and bottom panels of Fig.~\ref{fig:Summary_all_mass_ratios_spin}, respectively.}
\label{Tab:Summary_Stats_MCMC}
\end{table*}
